TCGM: An Information-Theoretic Framework for Semi-Supervised Multi-Modality Learning

Fusing data from multiple modalities provides more information to train machine learning systems. However, it is prohibitively expensive and time-consuming to label each modality with a large amount of data, which leads to a crucial problem of semi-supervised multi-modal learning. Existing methods suffer from either ineffective fusion across modalities or lack of theoretical guarantees under proper assumptions. In this paper, we propose a novel information-theoretic approach, namely \textbf{T}otal \textbf{C}orrelation \textbf{G}ain \textbf{M}aximization (TCGM), for semi-supervised multi-modal learning, which is endowed with promising properties: (i) it can utilize effectively the information across different modalities of unlabeled data points to facilitate training classifiers of each modality (ii) it has theoretical guarantee to identify Bayesian classifiers, i.e., the ground truth posteriors of all modalities. Specifically, by maximizing TC-induced loss (namely TC gain) over classifiers of all modalities, these classifiers can cooperatively discover the equivalent class of ground-truth classifiers; and identify the unique ones by leveraging limited percentage of labeled data. We apply our method to various tasks and achieve state-of-the-art results, including news classification, emotion recognition and disease prediction.

==> intro.tex <==
With the explosion of big data, many machine learning tasks have the access to multi-modal information. For example, medical images have different modalities such as sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography); perception data of autonomous driving have multiple modalities including camera, LIDAR, and RADAR sweeps. Learning with data from multiple modalities has the advantage to facilitate information fusion from different perspectives, hence, induce more robust models. For example, as shown in Figure \ref{fig:my_label}, to diagnose whether a patient has a certain disease or not, we can consult to its X-ray images, look into its medical records, or get results from clinical pathology. However, in many real applications, especially in some difficult ones (e.g. medical diagnosis), annotating such large-scale training data is prohibitively expensive and time-consuming. As a consequence, each modality of data may only contain a small proportion of labeled data from professional annotators, remaining a large proportion of unlabeled data, which leads to an essential and challenging problem of semi-supervised multi-modality learning: how to effectively utilize the information across different modalities with unlabeled data to train the classifier accurately? 


% For example, although it is easy to collect different modalities of examination data such as 3D images of sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography) for patients who are suspect of Alzheimer's Disease (AD), it is very difficult to have professional doctors label these large-scale examination data to train the diagnosis predictor.
% As a consequence, each modality of data may contain a large proportion of unlabeled data, which leads to an essential and challenging problem of semi-supervised multi-modality learning: how to effectively utilize the information across different modalities with unlabeled data to train the classifier accurately?

One type of existing solution to this problem is to adopt a co-training strategy to combine the information from different modalities \cite{blum1998combining,jones2005learning,balcan2005co,christoudias2006co,cheng2015semi}, which originates from Blum \etal \cite{blum1998combining} that iteratively augment samples with high confidence from one modality to another. Promising results as it achieves, the iterative scheme relies largely on the ``compatible" assumption that the conditional distributions for the data point labels in each modality are the same, which may not be satisfied in the real settings, as self-claimed in \cite{blum1998combining}. Another line of works learns a joint feature representation across multiple modalities in an unsupervised way \cite{ngiam2011multimodal, sohn2014improved, chandar2016correlational, wang2018efficient, chang2018scalable}, so that the small set of labeled data can be used to train a classifier to predict the label of the learned joint representation. However, such approaches cannot avoid learning a trivial solution that maps all the data points to the same representation and cannot learn a classifier for each modality.


\begin{figure}[h!]
    \centering
    \includegraphics[width=3in]{intersection.png}
    \caption{Multiple modalities are independent conditioning on the ground truth; Ground truth is the ``information intersection" of all of the modalities.}
    \label{fig:my_label}
\end{figure}

A common belief in multi-modality learning is that these modalities are conditionally independent, \ie, different modalities are independent given the ground truth label, as illustrated in Figure \ref{fig:my_label}. Many existing works have been built on such ``conditional independence" assumption, such as \cite{lewis1998naive,blum1998combining,dasgupta2002pac,leskes2005value}. For example, to diagnose whether a patient has a certain disease, there is some information related to the ground truth (e.g. whether there is a nodule) in a patient's X-ray image, and also some redundant information (e.g. the size of the patient's body), and so do the medical records and the clinical pathology. Conditioning on the ground truth, the redundant information from each modality is not necessarily correlated with each other. 
%Besides, Nigam \etal found that data has a natural division of features, which matches with the multi-modality scenario. 
%3D images of sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography) for patients who are suspect of Alzheimer's Disease (AD). Taking Alzheimer's Disease data as an example, sMRI data contains information about the volume of the hippocampus while PET data inform the degree of metabolism of the hippocampus in one's brain. An AD patient may suffer from both reduced volume and less metabolism degree of the hippocampus, but they are not necessarily correlated if the information of its labels is removed. 
In other words, the ground truth label can be regarded as the ``information intersection" across all modalities. To capture such information intersection, we propose an information-theoretic framework called TCGM (Total Correlation Gain maximization) for semi-supervised multi-modality learning, which aims to aggregate the knowledge from all modalities simultaneously. 

The spirit of our framework is to train the classifiers for each modality to maximize their total correlation gain, which measures the common information among all of the modalities, on the unlabeled subset of the dataset, while training them in the normal supervised way on the labeled subset. Furthermore, we devise an aggregator that employs all the modalities to forecast the label based on all of the modalities. It can be theoretically proved that, under the conditional independence assumption, the learned classifier for each modality is the Bayesian posterior classifier given each modality and the aggregator is the Bayesian posterior aggregator given all of the modalities. With the proposed TCGM, we target to solve the important mulit-modal learning problems, including the news classification with different three pre-processing steps as different modalites and the disease prediction of Alzheimer's Disease (AD) with the sMRI and PET modalities. We present the improved prediction power and interpretability in the experimental section to validate the efficacy of our method. On both tasks, our methods consistently outperform baseline methods in terms of prediction accuracy based on each single modality and prediction accuracy based on all modalities. In particular, we visualize some cases of AD whose label is difficult to be predicted via supervised learning with single modality; while our classifier based on single modality is able to correctly classify such hard samples, with more accurate learning of predicting the information intersection by maximizing total correlation among all modalities during training. 

The contributions of our paper can be summarized as follows: 1. We propose a novel information-theoretic approach TCGM for semi-supervised multi-modal learning. By maximizing the total correlation gain among all the modalities, the classifiers for different modalities cooperatively discover the information intersection across all the modalities - the ground truth. An aggregator is devised to employ all the modalities to forecast the label based on all of the modalities. 2. We theoretically proved that, under the conditional independence assumption, the learned classifier for each modality is the Bayesian posterior classifier given each modality and the aggregator is the Bayesian posterior aggregator given all of the modalities. 3. We solve the important mulit-modal learning problems, including the news classification and disease prediction and achieves the new state-of-the-art results.



==> intro_xw_risk.tex <==
%With the explosion of big data, many machine learning tasks have the access to multi-modal information. 
Learning with data from multiple modalities has the advantage to facilitate information fusion from different perspectives, hence, induces more robust models, compared with only using single modality. For example, as shown in Figure \ref{fig:my_label}, to diagnose whether a patient has a certain disease or not, we can consult to its X-ray images, look into its medical records, or get results from clinical pathology. However, in many real applications, especially in some difficult ones (e.g. medical diagnosis), annotating such large-scale training data is prohibitively expensive and time-consuming. As a consequence, each modality of data may only contain a small proportion of labeled data from professional annotators, leaving a large proportion unlabeled. This leads to an essential and challenging problem of semi-supervised multi-modality learning: \emph{how to effectively train accurate classifiers by aggregating unlabeled data of all modalities? }

%For example, medical images have different modalities such as sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography); perception data of autonomous driving have multiple modalities including camera, LIDAR, and RADAR sweeps. 



% For example, although it is easy to collect different modalities of examination data such as 3D images of sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography) for patients who are suspect of Alzheimer's Disease (AD), it is very difficult to have professional doctors label these large-scale examination data to train the diagnosis predictor.
% As a consequence, each modality of data may contain a large proportion of unlabeled data, which leads to an essential and challenging problem of semi-supervised multi-modality learning: how to effectively utilize the information across different modalities with unlabeled data to train the classifier accurately?

To achieve this goal, many methods have been proposed in the literature, which can be roughly categorized into two branches: (i) co-training strategy \cite{blum1998combining}; and (ii) learning joint representation across modalities in an unsupervised way \cite{ngiam2011multimodal, sohn2014improved}. These methods suffer from either strong assumptions or learning trivial solution. Specifically, the co-training strategy relies largely on the ``compatible'' assumption that the conditional distributions of the data point labels in each modality are the same, which may not be satisfied in the real settings, as self-claimed in \cite{blum1998combining}; while the latter branch of methods fails to capture the higher-order dependency among modalities, hence may end up in learning a trivial solution that maps all the data points to the same representation. 


\begin{figure}[h!]
    \centering
    \includegraphics[width=3.2in]{intersection.png}
    \caption{Multiple modalities are independent conditioning on the ground truth; Ground truth is the ``information intersection" of all of the modalities.}
    \label{fig:my_label}
\end{figure}

A common belief in multi-modality learning \cite{lewis1998naive,blum1998combining,dasgupta2002pac,leskes2005value} is that conditioning on ground truth label $Y$, these modalities are conditionally independent, as illustrated in Figure \ref{fig:my_label}. For example, to diagnose if one suffers from a certain disease, an efficient way is to leverage as many as modalities that are related to the disease, e.g., X-ray image, medical records and the clinical pathology. Since each modality captures the characteristics of the disease from different aspects, the information extracted from these modalities, in addition to the label, are not necessarily correlated with each other. This suggests that the ground truth label can be regarded as the ``information intersection'' across all the modalities, i.e., the amount of agreement shared by all the modalities. 






%For AD, to test if one suffers from AD, an efficient and reliable way is to scan one's brain to get the brain Structural magnetic resonance imaging (sMRI) and Positron emission tomography (PET). If a patient suffers from AD, both sMRI and PET shows abnormal pattern compared with normal controls (NC), however in different aspects. The sMRI, which extracts the information of structure of the brain, can show degeneration in some brain regions (e.g., two-side Hippocampus or medial temporal lobe); while the PET, which measures the chemical activity of one's brain, can show abnormal measurement of blood flow, oxygen use in corresponding regions. Since focusing on different aspects on a particular label (AD, Mild-Cognitive Impairment and NC), the information extracted from these two modalities are not necessarily correlated. Therefore, the label can be understood as the generating factor for sMRI and PET. 


% Conditioning on the ground truth, the redundant information from each modality is not necessarily correlated with each other. 
%Besides, Nigam \etal found that data has a natural division of features, which matches with the multi-modality scenario. 
%3D images of sMRI (structure Magnetic Resonance Imaging) and PET (Positron Emission Tomography) for patients who are suspect of Alzheimer's Disease (AD). Taking Alzheimer's Disease data as an example, sMRI data contains information about the volume of the hippocampus while PET data inform the degree of metabolism of the hippocampus in one's brain. An AD patient may suffer from both reduced volume and less metabolism degree of the hippocampus, but they are not necessarily correlated if the information of its labels is removed. 


Inspired by such an assumption and the fact that the \emph{Total Correlation} \cite{studeny1998multiinformation} can measure the amount of information shared by $M$ ($M \geq 2$) variables, in this paper, we propose Total Correlation Gain (TCG), which is a function of classifiers of all the modalities, as a surrogate goal for maximization of mutual information, in order to infer the ground-truth labels (i.e., information intersection among these modalities). 
Based on the proposed TCG, we devise an information-theoretic framework called \emph{\textbf{Total Correlation Gain Maximization}} (TCGM) for semi-supervised multi-modal learning.
By maximizing TCG among all the modalities, the classifiers for different modalities cooperatively discover the information intersection across all the modalities.
It can be proved that the optimal classifiers for such a Total Correlation Gain is equivalent to the Bayesian posterior classifiers given each modality under some permutation function. With further leverage of labeled data, we can identify the Bayesian posterior classifiers. Furthermore, we devise an aggregator that employs all the modalities to forecast the labels of data. 

We apply TCGM on news classification with three pre-processing steps as different modalities and the disease prediction of Alzheimer's Disease (AD) with the sMRI and PET modalities. On both tasks, our method consistently outperforms the baseline methods in terms of prediction accuracy based on each single modality and that based on all modalities. In particular, we visualize some cases of AD whose label is difficult to be predicted via supervised learning with single modality; while our jointly learned single modal classifier is able to correctly classify such hard samples. This is due to that the joint learning process of pursuing maximum information intersection induces the optimal Bayesian posterior classifier for each modality. \newline

%It can be theoretically proved that, under the conditional independence assumption, the learned classifier for each modality is the Bayesian posterior classifier given each modality and the aggregator is the Bayesian posterior aggregator given all of the modalities.


%And the aggregator is the Bayesian posterior aggregator given all of the modalities.

%propose an information-theoretic framework called TCGM (), which aims at pursuing the information intersection, i.e., the ground-truth label by maximizing the Total To capture such information intersection, we propose an  for semi-supervised multi-modality learning, which aims to aggregate the knowledge from all modalities simultaneously. 

%At a high level, the spirit of our framework is to train the classifiers for each modality to maximize their total correlation gain, which measures the common information among all of the modalities, on the unlabeled subset of the dataset, while training them in the normal supervised way on the labeled subset.



The contributions can be summarized as follows: 
\begin{itemize}
    \item We propose a novel information-theoretic approach TCGM for semi-supervised multi-modal learning. By maximizing the total correlation gain among all the modalities, the classifiers for different modalities cooperatively discover the information intersection across all the modalities - the ground truth. An aggregator is devised to employ all the modalities to forecast the label based on all of the modalities. 
    \item We theoretically proved that, under the conditional independence assumption, the learned classifier for each modality is the Bayesian posterior classifier given each modality and the aggregator is the Bayesian posterior aggregator given all of the modalities.
    \item  We solve the important mulit-modal learning problems, including the news classification and disease prediction and achieve the new state-of-the-art results.
\end{itemize}

==> method.tex <==
In this section, we formally describe the problem and introduce our method.

\paragraph{Problem statement} In the semi-supervised muli-modal learning senario, we have access to an unlabeled dataset $\mathcal{D}_u = \{x_i^{[M]}\}_i$ and a labeled dataset $\mathcal{D}_l = \{(x_i^{[M]}, y_i) \}_i$. Each label $y_i \in \mathcal{C}$, where $\mathcal{C}$ denotes the set of classes. Each datapoint $x_i^{[M]} := \{x_i^1, x_i^2, \dots, x_i^M | x_i^m \in \mathcal{X}^m \}$ consists of $M$ modalities, where $\mathcal{X}^m$ denotes the domain of the $m$-th modality. Data points in $\mathcal{D}_u$ are i.i.d. samples drawn from joint distribution $U_{X^{[M]}}(x^1, x^2, \dots, x^M) := \Pr[X^1 =x^1, X^2=x^2, \dots, X^M=x^M]$. Data points and labels in $\mathcal{D}_l$ are i.i.d. samples drawn from the joint distribution $U_{X^{[M]}, Y}(x^1, x^2, \dots, x^M, y) := \Pr[X^1 =x^1, X^2=x^2, \dots, X^M=x^M, Y=y]$. Now we want to train $M$ classifiers $h^{[M]} := \{h^1, h^2, \dots, h^M\}$ and an aggregator $\zeta$ such that $\forall m, h^m: \mathcal{X}^m \to \Delta_{\mathcal{C}}$ predicts the ground truth $y$ based on a $m$-th modality $x^m$ and $\zeta:\mathcal{X}^1\times\mathcal{X}^2\times\cdots\times\mathcal{X}^M \to \Delta_{\mathcal{C}}$ predicts the ground truth $y$ based on all of the modalities $x^{[M]}$.

 We assume that all of the modalities are independent conditioning on the ground truth, which is commonly assumed in the literature \cite{lewis1998naive,blum1998combining,dasgupta2002pac,leskes2005value}.

\begin{assumption}
\label{cond}
 $X^1, X^2, \dots, X^M$ are independent conditioning on $Y$, i.e., $\forall x^1, \dots, x^M$, 
\begin{align*}
    &\Pr[X^1=x^1, X^2 = x^2, \dots, X^M=x^M | Y=y] \\
    = &\Pi_m \Pr[X^m=x^m | Y=y].
\end{align*}

\end{assumption}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\textwidth]{whole.png}
    \caption{Our information-theoretic loss function $\mathcal{L}_{\text{MI}^f}$}
    \label{fig:overview}
\end{figure*}

Our training process is shown in Algorithm~\ref{alg: train}. We train the $M$ classifiers using the classic cross entropy loss on the labeled dataset and using our information-theoretic loss function $\mathcal{L}_{\text{MI}^f}$ on the unlabeled dataset alternately. As shown in Figure \ref{fig:overview}, by training with $\mathcal{L}_{\text{MI}^f}$, we reward the $M$ classifiers for their agreements on the same data point and punish the $M$ classifiers for their agreements on different data points. Intuitively, if we only reward them for their agreements, they may learn a trivial solution that classifies all data points into the same class. 

\paragraph{Classifiers $h^{[M]}$}
Each classfier $h^m(x^m;\Theta^m)$ is modeled by a deep neural network with parameters $\Theta^m$. For each modality $m$, we denote the set of all such classifiers by $H^m$ and $H^{[M]} := \{H^1, H^2, \dots, H^M\}$.

\paragraph{Aggregator $\zeta$} Given $M$ classifiers for each modality $h^{[M]}$ and a distribution $\mathbf{p}=(p_c)_c \in \Delta_\mathcal{C}$, an aggregator $\zeta$ is constructed by \[\zeta(x^{[M]}; h^{[M]}, \mathbf{p}) = \text{Normalize}(\left(\frac{\Pi_m h^m(x^m_i)_c}{(p_c)^{M-1}}\right)_c)\]
where $\text{Normalize}(\mathbf{v}) := \frac{\mathbf{v}}{\sum_c v_c}$ for all $\mathbf{v} \in \Delta_{\mathcal{C}}$.

\paragraph{Loss function $\mathcal{L}_{\text{CE}}$ for labeled data} We use the classic cross entropy loss for labeled data. Formally, for a batch of data points $\{x_i^{[M]}\}_{i=1}^B$ drawn from labeled data $\mathcal{D}_{l}$, the cross entropy loss $\mathcal{L}_{\text{CE}}$ for each classifier $h^m$ is defined as $\mathcal{L}_{\text{CE}}(\{(x_i^{[M]},y_i)\}_{i=1}^B; h^{m}) :=\frac{1}{B}\sum_i -\log(h^m(x^m_i)_{y_i})$.

\paragraph{Loss function $\mathcal{L}_{\text{MI}^f}$ for unlabeled data} For a batch of data points $\{x_i^{[M]}\}_{i=1}^B$ drawn from unlabeled data $\mathcal{D}_{u}$, our loss function $\mathcal{L}_{\text{MI}^f}$ is defined as:

\begin{align*}
    &\mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h^{[M]},\mathbf{p}) \\ 
    := &\frac{1}{B}\sum_{i} f^{\star}(f'(\frac{1}{\sum_c (\frac{\Pi_m (h^m(x^m_{i})_c )}{(p_c)^{M-1}})})) \\
    - &\frac{1}{B!/(B-M)!}\sum_{i_1\neq i_2 \neq \cdots \neq i_M} f'(\frac{1}{\sum_c(\frac{\Pi_m (h^m(x^m_{i_m})_c) }{(p_c)^{M-1}})})
\end{align*}


According to Lemma \ref{lemma:dual-multi}, the expectation of $-\mathcal{L}_{\text{MI}^f}$ is a lower-bound of the $f$-multi-information among $M$ modalities, \ie, $\forall h^{[M]},\mathbf{p}$, \[-\E_{ x_i^{[M]}\xleftarrow{\text{i.i.d.}} U_{X^{[M]}}} \mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h^{[M]},\mathbf{p}) \leq \text{MI}^f(X^{[M]}).\] 



\begin{definition}
[Bayesian posterior classifiers/aggregator] We define $h_{*}^{[M]}$ and $\zeta_{*}$ such that
\begin{align*}
    \forall m, h_{*}^{m}(x^m)_c &= \Pr[Y=c | X^m = x^m]; \\ \zeta_{*}(x^{[M]})_c &= \Pr[Y=c | X^{[M]} = x^{[M]}].
\end{align*}
 
We call them Bayesion posterior classifiers and Bayesion posterior aggragator.
\end{definition}

The Bayesian posterior classifiers are the minimizers of the expected cross entropy loss. It remains to show that the Bayesian posterior classifiers are also the minimizers of the expected $\mathcal{L}_{\text{MI}^f}$ for unlabeled data. We denote the prior of the ground truth labels by $\mathbf{p}^* = (\Pr[Y=c])_c$. 

\begin{theorem}
[Main theorem] $(h_{*}^{[M]}, \mathbf{p}^{*})$ is a minimizer of $\min_{\forall m, h^m\in H^m, \mathbf{p} \in \Delta_{ \mathcal{C}}} \mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h^{[M]},\mathbf{p})$, in other words, $\forall h^{[M]}\in H^{[M]}, \mathbf{p} \in \Delta_{ \mathcal{C}}$,
\begin{align*}
    &\E_{ x_i^{[M]}\xleftarrow{\text{i.i.d.}} U_{X^{[M]}}} \mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h^{[M]},\mathbf{p}) \\
    \geq &\E_{ x_i^{[M]}\xleftarrow{\text{i.i.d.}} U_{X^{[M]}}} \mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h_{*}^{[M]},\mathbf{p}^*),
\end{align*}
and the minimum \[\E_{ x_i^{[M]}\xleftarrow{\text{i.i.d.}} U_{X^{[M]}}} \mathcal{L}_{\text{MI}^f}(\{x_i^{[M]}\}_{i=1}^B; h_{*}^{[M]},\mathbf{p}^*) = -\text{MI}^f(X^{[M]}).\] Furthermore, $\forall x^{[M]}, \zeta_{*}(x^{[M]})=\zeta(x^{[M]};h_{*}^{[M]},\mathbf{p}^{*}).$
\end{theorem}
See proof in Appendix A.




==> prelim.tex <==
In this section, we provide some math tools and introduce the information measure we use, $f$-multi-information.

\paragraph{Notations} Given a random variable $W$, $\mathcal{W}$ denotes its realization space. Further, given a finite set $\mathcal{W}$, $\Delta_{\mathcal{W}}$ denotes the set of all distributions over $\mathcal{W}$. For every integer $M$, $[M]$ denotes the set $\{1,2,\dots,M\}$. For a vector $\mathbf{v}$, $v_i$ denotes the $i$-th element and $(v_i)_i$ denotes the whole vector. 

\begin{definition}[$f$-divergence \cite{csiszar2004information}] $\text{D}_f: \Delta_{\mathcal{W}} \times \Delta_{\mathcal{W}} \to \mathbb{R}$ is a measure of the difference between two distributions $p \in \Delta_{\mathcal{W}}$ and $q \in \Delta_{\mathcal{W}}$. It is defined to be \[D_f(p,q) = \sum_{w \in \mathcal{W}} q(w) f\left(\frac{p(w)}{q(w)}\right)\]
where $f: \mathbb{R}\to \mathbb{R}$ is a convex function and $f(1) = 0$.
\end{definition}
\begin{example}
Choosing $f(t) = t\log t$ as the convex function $f$, it becomes the Kullback–Leibler divergence \cite{csiszar2004information} $\text{D}_{\text{KL}}(p,q) = \sum_{w \in \mathcal{W}} p(w) \log\left(\frac{p(w)}{q(w)}\right)$.
\end{example}

\begin{definition}[Fenchel Duality \cite{rockafellar1966extension}] Given any convex function $f:\mathbb{R}\to \mathbb{R}$, its conjugate $f^{\star}:\mathbb{R}\to \mathbb{R}$ is defined as \[f^{\star}(x) = \sup_t (tx-f(t)).\]
\end{definition}


\begin{lemma}[Dual version of $f$-divergence \cite{nguyen2010estimating}]
\label{lemma:dual}
 \[\text{D}_f(p,q) \geq \sup_{g\in\mathcal{G}}( \E_{W\gets p} g(W) - \E_{W\gets q} f^{\star}(g(W)))\]
where $\mathcal{G}$ is a set of functions that maps $\mathcal{W}$ to $\mathbb{R}$. The equality holds 
if and only if $g(w) = g_{*}(w) =  f'\left(\frac{p(w)}{q(w)}\right)$, where $f'(t) := \frac{\mathrm{d}f(t)}{\mathrm{d}t}$.
\end{lemma}

Based on $f$-divergence, we propose a new information measure that measures the dependence among multiple random variables, $f$-multi-information.

\begin{definition}[$f$-multi-information]
Given $N$ random variables $W^{[N]}:=\{W^1, W^2, \dots, W^N\}$, let $U_{W^{[N]}}$ denote the joint distribution of $W^1, W^2, \dots, W^N$ and $V_{W^{[N]}}$ denote the product of the marginal distributions of $W^1, W^2, \dots, W^N$, \ie, 
\begin{align*}
    &U_{W^{[N]}}(w^1, w^2, \dots, w^N) \\
    = &\Pr[W^1=w^1, W^2=w^2, \dots, W^N=w^N],\\
    &V_{W^{[N]}}(w^1,w^2, \dots,w^N) \\
    = & \Pr[W^1=w^1]\Pr[W^2=w^2]\cdots\Pr[W^N=w^N].
\end{align*}
The $f$-multi-information among $W^{[N]}$ is defined as \[\text{MI}^f(W^{[N]}) := D_f(V_{W^{[N]}}, U_{W^{[N]}})\]
where $D_f$ is $f$-divergence. 
\end{definition}
\begin{example}
Choosing $f(t) = -\log t$ as the convex function $f$, it becomes the total correlation \cite{watanabe1960information} $\text{C}(W^{[N]})= \sum_{w^1,\dots, w^N} U_{W^{[N]}}(w^1,\dots ,w^N) \log {\frac  {U_{W^{[N]}}(w^1,\ldots ,w^N)}{V_{W^{[N]}}(w^1,w^2, \dots,w^N)}}$.
\end{example}

Table \ref{table:distinguishers} shows several common $f$-divergences and their corresponding $f'(t)$ and $f^{\star}(f'(t))$.

\begin{table}[!http]
\caption{Reference for common $f$-divergences and corresponding $f'(t)$ and $f^{\star}(f'(t))$}
\begin{center}
\begin{tabular}{cccc}
\toprule
    {$f$-divergence} & {$f(t)$} & {$f'(t)$} & {$f^{\star}(f'(t)$)} \\ \midrule\midrule
    KL-divergence & $t\log t$  & $1+\log t$ & $t$ \\ 
    \midrule
    reverse KL-divergence & $-\log t$  & $-\frac{1}{t}$ & $\log t - 1$ \\ 
    \midrule
    Pearson $\chi^2$-divergence  & $(t-1)^2$  & $2(t-1)$ & $t^2-1$ \\ 
    \bottomrule
\end{tabular}
\end{center}
\label{table:distinguishers}
\end{table}

\begin{definition}[Marginal-joint ratio]
We define the ratio between the product of the marginal distribution $V_{W^{[N]}}(w^1,w^2, \dots,w^N)$ and the joint distribution $U_{W^{[N]}}(w^1, w^2, \dots, w^N)$ as $\text{R}_{W^{[N]}}(w^1, w^2, \dots, w^N)$, \ie,
\begin{align*}
    &\text{R}_{W^{[N]}}(w^1, w^2, \dots, w^N) \\
:=&\frac{\Pr[W^1=w^1]\Pr[W^2=w^2]\dots\Pr[W^N=w^N]}{\Pr[W^1=w^1, W^2=w^2, \dots, W^N=w^N]}.
\end{align*}

\end{definition}


Lemma \ref{lemma:dual} directly implies a lower bound of $f$-multi-information.
\begin{lemma}[Dual version of $f$-multi-information] 
\label{lemma:dual-multi}
\begin{align*}
 & \text{MI}^f(W^{[N]}) \\
  \geq &\sup_{g\in\mathcal{G}}( \E_{K^{[N]}\gets V_{W^{[N]}}} g(K^1, \dots, K^N)\\
  - & \E_{K^{[N]}\gets U_{W^{[N]}}} f^{\star}(g(K^1, \dots, K^N)))  
\end{align*}
where $\mathcal{G}$ is the set of functions that maps $\mathcal{W}^1\times\mathcal{W}^2 \times \dots\times \mathcal{W}^N$ to $\mathbb{R}$. The equality holds if and only if $g(w^1, w^2, \dots, w^N) = g_{*}(w^1, w^2, \dots, w^N) = f'(\text{R}_{W^{[N]}}(w^1, w^2, \dots, w^N))$.
\end{lemma}

\pc{reviewer suggest that we should provide insights behind the definition of the loss function before developing our method}

